SCube: Instant Large-Scale Scene Reconstruction using VoxSplats

We present SCube, a novel method for reconstructing large-scale 3D scenes (geometry, appearance, and semantics) from a sparse set of posed images. Our method encodes reconstructed scenes using a novel representation VoxSplat, which is a set of 3D Gaussians supported on a high-resolution sparse-voxel scaffold. To reconstruct a VoxSplat from images, we employ a hierarchical voxel latent diffusion model conditioned on the input images followed by a feedforward appearance prediction model. The diffusion model generates high-resolution grids progressively in a coarse-to-fine manner, and the appearance network predicts a set of Gaussians within each voxel. From as few as 3 non-overlapping input images, SCube can generate millions of Gaussians with a 1024^3 voxel grid spanning hundreds of meters in 20 seconds. Past works tackling scene reconstruction from images either rely on per-scene optimization and fail to reconstruct the scene away from input views (thus requiring dense view coverage as input) or leverage geometric priors based on low-resolution models, which produce blurry results. In contrast, SCube leverages high-resolution sparse networks and produces sharp outputs from few views. We show the superiority of SCube compared to prior art using the Waymo self-driving dataset on 3D reconstruction and demonstrate its applications, such as LiDAR simulation and text-to-scene generation.

==> table/ablation.tex <==
\begin{wraptable}{r}{0.5\linewidth}
\vspace{-1.5em}
\begin{center}
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{ccc|cc}
\toprule
 \multirow{2}{*}{Resolution} & \multirow{2}{*}{$M$} & {\footnotesize Generative} & \multirow{2}{*}{PSNR$\uparrow$} & \multirow{2}{*}{LPIPS$\downarrow$} \\
 & & {\footnotesize Render} & & \\
\midrule
$256^3$ & 4 & & 18.58 & 0.62 \\
$1024^3$ & 1 & & 19.34 & 0.52 \\
$1024^3$ & 4 & & 19.34 & 0.48 \\
$1024^3$ & 4 & \checkmark & \textbf{21.71} & \textbf{0.36} \\
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-2mm}
\caption{\textbf{Ablation Study for Appearance Reconstruction}. 
}
\label{table:ablation}
\vspace{-1em}
\end{wraptable}

